PAVI: Plate-Amortized Variational Inference

Given some observed data and a probabilistic generative model, Bayesian inference aims at obtaining the distribution of a model's latent parameters that could have yielded the data. This task is challenging for large population studies where thousands of measurements are performed over a cohort of hundreds of subjects, resulting in a massive latent parameter space. This large cardinality renders off-the-shelf Variational Inference (VI) computationally impractical. In this work, we design structured VI families that can efficiently tackle large population studies. To this end, our main idea is to share the parameterization and learning across the different i.i.d. variables in a generative model -symbolized by the model's plates. We name this concept plate amortization, and illustrate the powerful synergies it entitles, resulting in expressive, parsimoniously parameterized and orders of magnitude faster to train large scale hierarchical variational distributions. We illustrate the practical utility of PAVI through a challenging Neuroimaging example featuring a million latent parameters, demonstrating a significant step towards scalable and expressive Variational Inference.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} In \cref{sec:archi} we introduce the our plate-amortized architecture, in \cref{sec:training} our stochastic training scheme, and in \cref{sec:exps} we show how the combination of the 2 results in the fast convergence of efficiently parameterized variational distributions
  \item Did you describe the limitations of your work?
    \answerYes{} In \cref{sec:exp_scaling} we illustrate the parameter and speed trade-offs entitled by our various schemes, and we further detail in our supplemental material the performance gaps theoretically implied by plate amortization 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{} Given the generality of the approach proposed, we did not find it has any negative impact intrinsic to it.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} the Bayesian framework is presented thoroughly in \cref{sec:archi}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} as part of the code in our supplemental material
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} as part of a dedicated section in our supplemental material
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} error bars visible in \cref{fig:convergence_speed} and \cref{fig:scaling}. Errors are standard deviations calculated over a hundred runs of the algorithms.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} In a dedicated paragraph at the beginning of our experiments in \cref{sec:exps}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} see at the beginning of \cref{sec:exps} and in \cref{sec:exp_fMRI}
  \item Did you mention the license of the assets?
    \answerNo{} We only used completely public libraries which report their licenses in their documentation.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} as part of the Human Connectome Project dataset collection
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{} data from the Human Connectome Project is strongly anonymized
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
